Popular decision tree algorithms are provably noise tolerant

Using the framework of boosting, we prove that all impurity-based decision tree learning algorithms, including the classic ID3, C4.5, and CART, are highly noise tolerant. Our guarantees hold under the strongest noise model of nasty noise, and we provide near-matching upper and lower bounds on the allowable noise rate. We further show that these algorithms, which are simple and have long been central to everyday machine learning, enjoy provable guarantees in the noisy setting that are unmatched by existing algorithms in the theoretical literature on decision tree learning. Taken together, our results add to an ongoing line of research that seeks to place the empirical success of these practical decision tree algorithms on firm theoretical footing.

==> gray.tex <==

\gray{
\section{Overview of the whole thing} 

\subsection{Cast of characters} 
\begin{enumerate} 
\item Target function $f : X \to \bits$
\item Distribution $\mathcal{D}$ over domain $X$. 
\item Set of allowable internal nodes of tree $\mathcal{H}$.  For example, $\mathcal{H} = \{ x_1,\ldots,x_d\}$.\lnote{If we are submitting to an ML venue, let's use $d$ instead of $n$ for dimension.}  A more expressive set $\mathcal{H}$ allows for more expressive trees, but one then sacrifices interpretability. 
\item Impurity function $G : [-1,1]\to [0,1]$. 
\item The tree $\TopDown_{\mathcal{H},G}(f,\mathcal{D},t)$,  where $t \in \N$ is a size parameter.   This is the tree that TopDown builds when trained on $(\bx,f(\bx))$ where $\bx \sim \mathcal{D}$, and we iteratively split the leaf that maximizes $G$-impurity gain until we get a size-$t$ tree, and then we round the leaves.  
\end{enumerate} 


\subsection{Kearns Mansour} 

DTs can be viewed as {\sl distribution-specific} boosters 

\begin{definition}[Induced distributions]
Given a distribution $\mathcal{D}$ over $X$ and a set $\mathcal{H}$ of functions $X \to \bits$, we say that $\mathcal{D}'$ is a {\sl conditional distribution of $\mathcal{D}$ induced by $\mathcal{H}$} if $\mathcal{D}'$ can be expressed as [...]
\end{definition} 

Example where $\mathcal{D}$ is product and $\mathcal{H}$ is set of singleton variables. Conditional distributions remain product, and do not depend on target function.  Contrast with Adaboost. 


\begin{definition}[Distribution-specific weak learning assumption]\lnote{Kearns--Mansour describe this as ``$f$ satisfying the weak learning assumption w.r.t.~$\mathcal{H}$", but isn't it more natural to think of it as $\mathcal{H}$ satisfying the weak learning assumption w.r.t.~$f$?} 
Let $f : X \to \bits$ be a target function, $\mathcal{D}$ be a distribution over $X$, $\mathcal{H}$ be a set of allowable internal nodes, and $\gamma \in (0,1)$.  We say that $\mathcal{H}$ satisfies the $\gamma$-weak learning assumption with respect to $f$ and $\mathcal{D}$ if for every conditional distribution $\mathcal{D}'$ of $\mathcal{D}$ induced by $\mathcal{H}$, there exists $h\in \mathcal{H}$ such that [...]
 \end{definition} 
 
 
 \begin{theorem}[Kearns Mansour] 
 Suppose $\mathcal{H}$ satisfies the $\gamma$-weak learning assumption with respect to $f$ and $\mathcal{D}$.  Then growing $\TopDown_{\mathcal{H},G}(f,\mathcal{D},t)$ to size $t =$ [...] suffices to guarantee a decision tree hypothesis for $f$ with error $\le \eps$ w.r.t.~$\mathcal{D}$. 
 \end{theorem} 

Notable feature of this result is that the size of the tree is dimension independent. 

\subsection{Our hoped-for result} 

Difference with Kearns--Mansour highlighted in violet 

\begin{theorem} 
Suppose $\mathcal{H}$ satisfies the $\gamma$-weak learning assumption with respect to $f$ and $\mathcal{D}$.  \violet{Let $\wh{f}$ and $\wh{\mathcal{D}}$ be $\eta$-corruptions of $f$ and $\mathcal{D}$ where $\eta \le O(\eps\gamma)$}.  Then growing $\TopDown_{\mathcal{H},G}(\violet{\wh{f},\wh{\mathcal{D}}},t)$ to size $t = $ [...] suffices to guarantee a decision tree hypothesis for $f$ with error $\violet{\le 2\eta + \eps}$ w.r.t.~$\mathcal{D}$. 
\end{theorem} 

So I guess the point is that we only assume that $\mathcal{H}$ satisfies the weak learning assumption w.r.t.~the clean target $f$ and distribution $\mathcal{D}$---exactly the same assumption as in Kearns--Mansour. And yet, even if TopDown is trained on the corrupted $\wh{f}$ and $\wh{\mathcal{D}}$, it still succeeds. \lnote{Can we handle adaptive adversaries?}  

The crux of Kearns and Mansour's analysis is that TopDown makes good progress with every split.  No longer the case in the noisy setting. 


\paragraph{Optimality of our parameters} 

\begin{enumerate} 
\item error $2\eta + \eps$ is information-theoretically optimal. 
\item Noise rate $\eta \le O(\eps\gamma)$.  Optimal even for agnostic noise?  ``Approximate resilience, monotonicity, and the complexity of agnostic learning".  
\item Size of tree $\exp(1/\eps^2\gamma^2)$.   Best one can hope for is $\exp(\log(1/\eps)/\gamma^2)$. 
\end{enumerate} 

\subsection{Comparison with prior work} 

Our work unifies and strengthens several existing results: 
\begin{enumerate} 
\item Prior to our work, Kearns--Mansour was the only result that gave provable guarantees for TopDown without distributional or feature assumptions.  Our main result shows that these provable guarantees continue to hold even under the adversarial noise. 
\item Lots of work on boosting in the presence of noise, but none of these handle adversarial corruptions of both examples and labels. 
\item A number of papers giving provable guarantees under the assumption that $\mathcal{D}$ is product or uniform.  Most relevant for us are BLT-ICML and BLT-ICALP. 
\begin{enumerate} 
\item A variety of ways to learn decision trees in the presence of adversarial noise in time $d^{O(\log s)}$: $L_1$ and $L_2$ polynomial regression.  But these are not proper and do not achieve the information-theoretically optimal error of $2\eta + \eps$.  BLT recently gave a proper algorithm that runs in time $d^{O(\log s)}$ and achieves error $2\eta +\eps$. 
\item Note that the runtime of these algorithms, $d^{O(\log s)}$, is superpolynomial once $s = \omega_d(1)$. There's a good reason for this.  Even in the noiseless setting, all SQ algorithms require time $d^{\Omega(\log s)}$.  Our work shows that this barrier can be circumvented for monotone functions: our runtime is $\poly(d)\cdot s^{O(\log s)}$, which is $\poly(d)$ for $s$ as large as $2^{\Omega(\sqrt{\log d})}$.  
\item BLT-ICML's algorithm for monotone decision trees also runs in $\poly(d)\cdot s^{O(\log s)}$ time, but only handles adversarial label noise.  Our noise model is strictly more challenging, allowing corruptions of examples and labels, and not requring the corrupted function to remain monotone. 
\end{enumerate} 
\end{enumerate} 

\newpage 



\section{Introduction}

Top-down decision tree heuristics used in practice are noise tolerant boosting algorithms. Kearns and Mansour had shown that they can be viewed as boosting algorithms. Formal evidence that DT heuristics are tolerant to noise in the data -- this has been observed to hold in practice, but we give the first theoretical justification using the framework of boosting. 

\section{Preliminaries}
 
 \begin{enumerate}
     \item Let $\mcH$ be our hypothesis class of boolean functions from $\mcX$ to $\{-1, +1\}$.
     
     \item  For any distribution $\mcD$ over $\mcX$ and boolean functions $f,h : \mcX \to \{-1, 1\}$ define
     
     \begin{align*}
        \error_\mcD(f) &= \min \left\{\Pr_\mcD[f(X) = 1], 1 - \Pr_\mcD[f(X) = 1]\right\} \\
        \Var_\mcD(f) &= 4\Pr_\mcD[f(X) = 1](1 - \Pr_\mcD[f(X) = 1]) \\
        \dist_\mcD(f, h) &= \Pr_\mcD[f(X) \neq h(X)] \\    
     \end{align*}
     
     \item Given a distribution $\mcD$ over $\mcX$ and a decision tree $\mcT$, for any leaf $\ell$ in the tree, we denote $\mcD_\ell$ to the conditional distribution over $\mcX$ induced by $\mcD$ on the inputs that reach $\ell$.
     
     \item Given a distribution $\mcD$ over $\mcX$ and a target function $f$, we denote ${\mcD^{\mathrm{Bal}}}$ to be a rebalanced version of $\mcD$ that gives equal weight to positive and negative examples, i.e. $\Pr_{{\mcD^{\mathrm{Bal}}}}[f(X) = 1] = 1/2$. Specifically, let $p = \Pr_{\mcD}[f(X) = 1]$. Then for $x \in \mcX$:
     
     \[
        {\mcD^{\mathrm{Bal}}}(x) = \begin{cases}
    \mcD(x)/2 p \quad &\text{if } f(x) = 1 \\
    \mcD(x)/2(1 - p) \quad &\text{if } f(x) = -1.
    \end{cases}
    \]
     
 \end{enumerate}
 
 
 
\begin{fact}\label{fact:errvar}
For a function $f : \mcX \to \{-1, 1\}$ and any distribution $\mcD$ over $\mcX$,

\begin{equation}
    \frac{\Var_{\mcD}(f)}{4} \leq \error_\mcD(f) \leq \frac{\Var_{\mcD}(f)}{2}.
\end{equation}
\end{fact}





\subsection{Noise models} 

TODO: Formalize agnostic v1 and v2, and nasty v1 and v2. 



\begin{itemize}

\item \textbf{Agnostic v1}.

    Choose $\tilde{X} \subseteq X$ s.t. $\Pr_\mcD[x \in \tilde{X}] \leq \eta$.
    
    \[
        g(x) = 
            \begin{cases}
                f(x)   &\text{if $x \in X - \tilde{X}$} \\
                \lnot f(x)   &\text{if $x \in \tilde{X}$}
            \end{cases}
    \]    
    

\item \textbf{Nasty v1}.

Choose $\tilde{X} \subseteq X$ s.t. $\Pr_\mcD[x \in \tilde{X}] \leq \eta$.

    \[
        (x, f(x)) \to  
            \begin{cases}
                (x, f(x))   &\text{if $x \in X - \tilde{X}$} \\
                (x', y')   &\text{if $x \in \tilde{X}$} \\
            \end{cases}
    \]
        
    
\item \textbf{Agnostic v2}.

Sample $\{(x_i, f(x_i))\}_{i=1}^N$. Adversary gets to pick up to $\eta$ fraction of these points to flip the label of.



    
\item \textbf{Nasty v2}.

Sample $\{(x_i, f(x_i))\}_{i=1}^N$. Adversary gets to pick $\eta$ fraction of these points to remove and replace with anything.


\item \textbf{Agnostic (alt)}.

Let $g$ be a function (possibly randomised) s.t. $\dist(f, g) \leq \eta$. Note this distance is both w.r.t the distribution $\mcX$ and any internal randomisation of $g$.  

Return points labelled with $g$ i.e. samples $(x, g(x))$ where $x \sim \mcD$. This covers both the Agnostic v1 case (when $g$ is deterministic) and also usual streaming noise models like:

    \[
        (x, f(x)) \to  
            \begin{cases}
                (x, f(x))   &\text{w.p. $(1 - \eta)$} \\
                (x, y')   &\text{w.p. $\eta$} \\
            \end{cases}
    \]
    
However, this alt. model is weaker than Agnostic v2 since in v2, the adversary can adaptively pick $g$ tailored for the specific sample.


\end{itemize}



\subsection{Top-Down Decision Tree Algorithms and Boosting}
 
 TODO: introduce notation about DTs, top-down DT algorithms, and the boosting framework
 
 We use the weak learning assumption introduced by \cite{km99boosting}:
 
 \begin{definition}[Weak Learning Assumption]
    Let $\gamma \in (0, 1]$ be called the advantage and $f : \mcX \to \{-1, 1\}$ be a boolean function. We say $f$ satisfies the $\gamma$-weak learning assumption with respect to the hypothesis class $\mcH$ if, for any distribution $\mcD$ over $\mcX$, there exists a hypothesis $h \in \mcH$ s.t. $\E_{\mcD}[f(X) h(X)] \geq \gamma$. 
 \end{definition}
 
 Note that this definition is equivalent to that of \cite{km99boosting} since a correlation of at least $\gamma$ is equivalent to $\Pr_\mcD[f(X) \neq h(X)] \leq 1/2 - \gamma/2$.

\section{Noise Tolerance of Top-down Decision Tree Algorithms: Agnostic noise}


We focus on the agnostic (v1 + alt) setting. \anote{TODO: Reference other section if we are able to show v1 = v2}

\begin{lemma}\label{lem:noisy_wla}
    Let $\mcD$ be a distribution over $\mcX$ and let $f : \mcX \to \{-1, 1\}$ be a boolean function that satisfies the $\gamma$-weak learning assumption for $\mcH$. Further, suppose an adversary is allowed to corrupt up to $\eta$ fraction of labels by creating a new malicious function $\widehat{f}$ such that $\dist_\mcD(f, \widehat{f}) \leq \eta$.
    
    
    
    Then there exists an $h \in \mcH$ s.t.
    
    \begin{equation}
        \E_{\mcD}[\widehat{f}(X) h(X)] \geq \gamma - 2\eta.
    \end{equation}
    
    
    % For any other function $\widehat{f} : \mcX \to \{-1, 1\}$ such that $\Pr_{\mcD}[f(X) \neq \widehat{f}(X)] \leq \eta$, we have that $\widehat{f}$ satisfies the $(\gamma - 2\eta)$-weak learning assumption for $\mcH$.
\end{lemma}
\begin{proof}
 Since $f$ satisfies the $\gamma$-weak learning assumption for $\mcH$, there exists an $h \in \mcH$ such that $\E_{\mcD}[f(X) h(X)] \geq \gamma$. The adversary can change $\eta$ fraction of values of $f$ in $\widehat{f}$, and because
 
 \[
 \E_{\mcD}[f(X) h(X)] = \Pr_{\mcD}[f(X) = h(X)] - \Pr_{\mcD}[f(X) \neq h(X)],
 \]
 
 the worst case is if the adversary flips as many points as it can where $f(X) = h(X)$. This would remove $\eta$ mass from $\Pr_{\mcD}[f(X) = h(X)]$ and add $\eta$ mass to $\Pr_{\mcD}[f(X) \neq h(X)]$, so that 
 
  \begin{align}
      \E_{\mcD}[\widehat{f}(X) h(X)] &= \Pr_{\mcD}[\widehat{f}(X) = h(X)] - \Pr_{\mcD}[\widehat{f}(X) \neq h(X)] \\
      &= \paren{\Pr_{\mcD}[f(X) = h(X)] - \eta} - \paren{\Pr_{\mcD}[f(X) \neq h(X)] + \eta} \\
      &= \E_{\mcD}[f(X) h(X)] - 2\eta \\ 
      &\geq \gamma - 2\eta.
  \end{align}
\end{proof}

Lemma \ref{lem:noisy_wla} lets us use the fact that if there exists a function $h$ that has high correlation with $f$, then this same $h$ will also have high correlation when $\eta$ fraction of labels are corrupted. 




The following lemma from \cite{km99boosting} uses the existence of a function correlated with $f$ on a balanced distribution to lower bound the purity gain caused by splitting a leaf. 

\begin{lemma}[Kearns and Mansour]\label{lem:km_gain}
Let $f : \mcX \to \{-1, 1\}$ be a boolean function, $\mcT$ be a decision tree, $\ell$ be a leaf in this tree, and consider $G(p) = 4p(1-p)$ as the impurity function used by \BuildTD. We use $\mcD_\ell$ to denote the distribution over $\mcX$ at this leaf. Suppose there exists an $h : \mcX \to \{-1, 1\}$ such that $\E_{{\mcD^{\mathrm{Bal}}_\ell}}[f(X) h(X)] \geq \gamma$, for $\gamma \in (0, 1]$. Then,

\begin{equation}
    \Delta_{f}(\mcT, \ell, h) \geq \gamma^2 \Var_{\mcD_\ell}(f)^2,
\end{equation}

where $\Delta_{f}(\mcT, \ell, h)$ denotes the (unweighted) purity gain caused by splitting at leaf $\ell$ with function $h$.
\end{lemma}

\begin{proof}
TODO follows from KM
\end{proof}





\begin{lemma}\label{lem:noisy_wla_gain}
Let $f : \mcX \to \{-1, 1\}$ be a boolean function that satisfies the $\gamma$-weak learning assumption for $\mcH$, let $\mcT$ be a decision tree, and $\ell$ be a leaf in this tree. We use $\mcD_\ell$ to denote the distribution over $\mcX$ at this leaf. Consider a malicious $\widehat{f} : \mcX \to \{-1, 1\}$ such that $\dist_{\mcD_\ell}(f, \widehat{f}) \leq \eta_\ell$, where $\eta_\ell$ is the noise rate at this leaf.
 
 
Then, as long as $\gamma\Var_{\mcD_\ell}(\widehat{f}) > 4 \eta_\ell$, for the impurity function $G(p) = 4p(1-p)$, there exists an $h : \mcX \to \{-1, 1\}$ such that 

\begin{equation}
    \Delta_{\widehat{f}}(\mcT, \ell, h) \geq \paren{\gamma\Var_{\mcD_\ell}(\widehat{f}) - 4 \eta_\ell}^2.
\end{equation}

\end{lemma}

\begin{proof}
Let $\widehat{p}_\ell = \Pr_{\mcD_\ell}[\widehat{f}(X) = 1]$ and consider the balanced distribution w.r.t $\widehat{f}$: 

\[
{\mcD^{\mathrm{Bal}}_\ell}(x) = \begin{cases}
    \mcD_\ell(x)/2 \widehat{p}_\ell \quad &\text{if } \widehat{f}(x) = 1 \\
    \mcD_\ell(x)/2(1 - \widehat{p}_\ell) \quad &\text{if } \widehat{f}(x) = -1.
    \end{cases}
\]

If $\dist_{\mcD_\ell}(f, \widehat{f}) \leq \eta_\ell$, then  the most the noise rate can be amplified on the balanced distribution is by a factor of $1/2\min(\widehat{p}_\ell, 1 - \widehat{p}_\ell)$ corresponding to all the noisy labels being in the minority class. It follows from this that that $\dist_{{\mcD^{\mathrm{Bal}}_\ell}}(f, \widehat{f}) \leq 2\eta_\ell/\Var_{\mcD_\ell}(\widehat{f})$.

Applying Lemma \ref{lem:noisy_wla} with the balanced distribution ${\mcD^{\mathrm{Bal}}_\ell}$ and the noise rate $2\eta_\ell/\Var_{\mcD_\ell}(\widehat{f})$ gives us an $h \in \mcH$ such that

    \begin{equation}
        \E_{{\mcD^{\mathrm{Bal}}_\ell}}[\widehat{f}(X) h(X)] \geq \gamma - \frac{4\eta_\ell}{\Var_{\mcD_\ell}(\widehat{f})}.
    \end{equation}
    
The assumption that $\gamma\Var_{\mcD_\ell}(\widehat{f}) > 4 \eta_\ell$ guarantees that the advantage of $h$ on $\widehat{f}$ w.r.t ${\mcD^{\mathrm{Bal}}_\ell}$ is positive. Thus $h$ satisfies the conditions for Lemma \ref{lem:km_gain}, giving the desired result:

\begin{align}
    \Delta_{\widehat{f}}(\mcT, \ell, h) &\geq \paren{\gamma - \frac{4 \eta_\ell}{\Var_{\mcD_\ell}(\widehat{f})}}^2 \Var_{\mcD_\ell}(\widehat{f})^2 \\ 
    &= \paren{\gamma\Var_{\mcD_\ell}(\widehat{f}) - 4 \eta_\ell}^2.
\end{align}



\end{proof}






\begin{theorem}[Top-Down decision tree algorithms are noise-tolerant]

Let $\mcD$ be a distribution over $\mcX$ and let $f : \mcX \to \{-1, 1\}$ be a boolean function that satisfies the $\gamma$-weak learning assumption for $\mcH$. We consider $G(p) = 4p(1-p)$ to be the impurity function used by \BuildTD. Furthermore, let $\eta$ be a noise parameter s.t. an adversary is allowed to corrupt $\eta$ fraction of labels\anote{Add details of noise model and how much noise we allow}, by creating a new malicious function $\widehat{f}$ with $\dist_{\mcD}(f, \widehat{f}) \leq \eta$. 

Then, after $S \geq e^{c /(\gamma^2 \eps^2)}$ steps, the decision tree $\mcT$ output by $\BuildTD_{\mcD}(\widehat{f}, S)$ satisfies

\begin{equation}
    \dist_\mcD(\widehat{f}, \mcT) \leq 2\eta/\gamma + \eps.
\end{equation}

so that 

\begin{equation}
    \dist_\mcD(f, \mcT) \leq \eta + 2\eta/\gamma + \eps.
\end{equation}

\end{theorem}

\begin{proof}
Let $\mcT^\circ$ be the size-$(t+1)$ partial tree built by \BuildTD after $t$ iterations. Suppose we are not done, so that $\dist_\mcD(\widehat{f}, \mcT^\circ) > 2\eta/\gamma + \eps$ and let $\ell^*, h^*$ be the leaf and labelling function that is split in the $(t+1)$-st iteration. We claim that

\begin{equation}
    \Delta_{\widehat{f}}(\mcT^\circ, \ell^*, h^*) \geq \frac{4\eps^2 \gamma^2}{(t+1)}.
    % &= \paren{\gamma\Var_{\mcD_\ell}(\widehat{f}) - 4 \eta_\ell}^2.
\end{equation}

By assumption, since  $\dist_\mcD(\widehat{f}, \mcT^\circ) > 2\eta/\gamma + \eps$, this implies that $\eps \gamma < \gamma \dist_\mcD(\widehat{f}, \mcT^\circ) - 2\eta $, which gives:

\begin{align*}
    \eps \gamma  
        &< \gamma \dist_\mcD(\widehat{f}, \mcT^\circ) - 2 \eta  &\\
        &= \sum_{\text{leaves } \ell \in \mcT^\circ} w(\ell) \paren{\gamma  \error_{\mcD_{\ell}}(\widehat{f}) - 2\eta_\ell}  &\text{(by definition)}\\
        &\leq \frac{1}{2} \sum_{\text{leaves } \ell \in \mcT^\circ} w(\ell) \paren{\gamma  \Var_{\mcD_{\ell}}(\widehat{f}) - 4\eta_\ell}  &\text{(by Fact \ref{fact:errvar})}\\
        &\leq \frac{1}{2} \sum_{\text{leaves } \ell \in \mcT^\circ} w(\ell) \relu\paren{\gamma  \Var_{\mcD_{\ell}}(\widehat{f}) - 4\eta_\ell}  &\text{($\relu(x) \geq x$)}
\end{align*}

This gives:

\begin{align*}
    4 \eps^2 \gamma^2 
        &\leq \paren{\sum_{\text{leaves } \ell \in \mcT^\circ} w(\ell) \relu\paren{\gamma  \Var_{\mcD_{\ell}}(\widehat{f}) - 4\eta_\ell}}^2  &\\
        &\leq \sum_{\text{leaves } \ell \in \mcT^\circ} w(\ell) \paren{\relu\paren{\gamma  \Var_{\mcD_{\ell}}(\widehat{f}) - 4\eta_\ell}}^2   &\text{(Jensen's Inequality)}
\end{align*}

This implies there must be some leaf $\ell^*$ s.t. 

\begin{align}
w(\ell^*)\paren{\relu\paren{\gamma  \Var_{\mcD_{\ell^*}}(\widehat{f}) - 4\eta_\ell^*}}^2 > \frac{4\eps^2\gamma^2}{(t+1)}.
\end{align}

% \begin{equation}
% w(\ell^*)\paren{\gamma  \Var_{\mcD_{\ell^*}}(\widehat{f}) - 4\eta_\ell^*}^2 > \frac{4\eps^2\gamma^2}{(t+1)}.
% \end{equation}

This guarantees that for $\ell^*$, we have $\gamma  \Var_{\mcD_{\ell^*}}(\widehat{f}) > 4\eta_\ell^*$. So, by Lemma \ref{lem:noisy_wla_gain}, we know there exists an $h \in \mcH$ s.t.

\begin{align}
w(\ell^*) \Delta_{\widehat{f}}(\mcT, \ell^*, h) &\geq w(\ell^*) \paren{\gamma\Var_{\mcD_{\ell^*}}(\widehat{f}) - 4 \eta_{\ell^*}}^2 \\
&\geq w(\ell^*) \paren{\relu\paren{\gamma\Var_{\mcD_{\ell^*}}(\widehat{f}) - 4 \eta_{\ell^*}}}^2 \\
&\geq \frac{4\eps^2\gamma^2}{(t+1)}.
\end{align}


Since Top-Down picks a leaf and hypothesis that maximises purity gain, we are guaranteed that, at each iteration $t$, we reduce the impurity by at least $4\eps^2\gamma^2/(t+1)$. This means after $S \geq e^{c/\gamma^2\eps^2}$ iterations, we will be done. 

TODO: flesh out.

\end{proof}



\section{Relationship between agnostic noise and nasty noise} 


TODO: In the distribution free setting, prove that agnostic v1 and nasty v1 are equivalent. \\



TODO: Even in distribution-specific setting, for SQ algorithms, nasty v1 and nasty v2 are equivalent (ditto agnostic v1 and agnostic v2). 

SQ model:  underlying $\mcD$, make poly SQs to get $\Ex_\mcD[\chi] \pm \eps$.

v1 agnostic:
each sq is correlation.
adv chooses g eta-close to f and get SQs w.r.t g. 

Alg. guaranteed to return good hypothesis given access to SQs from g.


v2 agnostic:





Therefore the boosting results in the previous section extend to nasty v2. 

\section{Learning monotone decision trees in the presence of nasty noise}

Uniform distribution.  Goal is to handle nasty v2? 
}
